Joint Power and User Grouping Optimization in Cell-Free Massive MIMO Systems

To relieve the stress on channel estimation and decoding complexity in cell-free massive multiple-input multiple-output (MIMO) systems, user grouping problem is investigated in this paper, where access points (APs) based on time-division duplex (TDD) are considered to serve users on different time resources and the same frequency resource. In addition, when quality of service (QoS) requirements are considered, widely-used max-min power control is no longer applicable. We derive the minimum power constraints under diverse QoS requirements considering user grouping. Based on the analysis, we formulate the joint power and user grouping problem under QoS constraints, aiming at minimizing the total transmit power. A generalized benders decomposition (GBD) based algorithm is proposed, where the primal problem and master problem are solved iteratively to approach the optimal solution. Simulation results demonstrate that by user grouping, the number of users served in cell-free MIMO systems can be as much as the number of APs without increasing the complexity of channel estimation and decoding. Furthermore, with the proposed user grouping strategy, the power consumption can be reduced by 2-3 dB compared with the reference user grouping strategy{, and by 7 dB compared with the total transmit power without grouping.

==> CHANGELOG <==
Changes made in the caption package bundle
==========================================

Please note that this document does not reflect bugfix-releases, and that the dates given are the dates of the release w/o bugfixes.

If you are interested in a complete changelog -- including bugfixes -- process the dtx files with \RecordChanges and \PrintChanges.


caption package
---------------

v1.0 (1994/10/27)
- 1st published version

v1.1 (1994/11/03)
- New option `centerlast'

v1.2 (1994/11/28)
- Support of the `float' package added

v1.3 (1995/01/09)
- Support of \captionlabelfont in subcaptions added

v1.4 (1995/01/30)
- New option `nooneline'

v2.0 (caption2, 1995/10/09)
- New experimental version with many new commands and features
- Support of the `longtable' package added

v2.1 (caption2, 2002/02/26)
- Adapted to version 2.1 of the subfigure package
- New options for interaction with other packages (float,...)
- New command \normalcaptionparams
- New commands \captionof and \captionof*
- New ifs \ifcaptionlabel and \ifignoreLTcapwidth
- \realcaptionwidth renamed to \captionlinewidth

v2.2 (caption2, 2007/04/06)
- Internal change: Uses the caption3 kernel now

v3.0 (2003/12/20)
- Completely rewritten in cooperation with Frank Mittelbach and Steven Cochran

v3.1 (2007/09/01)
- Improved compatibility to supported document classes and packages, but decreased compatibility to non-supported document classes and packages
- Support of the AMS & SMF document classes added
- Support of the `beamer' document class added
- Support of the `KOMA-Script' document classes added
- Support of the `floatflt' package added
- Support of the `fltpage' package added
- Support of the `picinpar' package added
- Support of the `picins' package added
- Support of the `threeparttable' package added
- Support of the `wrapfig' package added
- Support of the `xtab' package added
- Check against incompatible `ftcap' package added
- Check against incompatible `nonfloat' package added
- Check against incompatible `topcapt' package added
- Does not process global options anymore to avoid conflicts with document class options
- New option compatibility=
- New options font+=, labelfont+= & textfont+=
- New options hypcap= & hypcapspace=
- New options list= and listformat=
- New option options=
- New options figurewithin= and tablewithin=
- Starred variant of option margin*= added
- Starred variant of option style*= added
- Starred variant of option type*= added
- Font options `normal', `normalcolor', `color', `normalfont' & `stretch' added
- Default position changed from `bottom' to `auto'
- New command \DeclareFloatingEnvironment resp. \DeclareCaptionType
- New command \DeclareCaptionListFormat
- New command \captionlistentry
- Starred variant of \clearcaptionsetup added
- Optional argument added to \clearcaptionsetup
- Starred variant of \ContinuedFloat added
- \captionsetup{...} inside longtables added
- \captionsetup[singleline]{...} added
- A \label before \caption will result in warning "\label before \caption ignored"
- The counters lofdepth & lotdepth are supported now
- Label formats have three arguments now
- Optional argument added to \DeclareCaptionFormat; "format=plain" removed from single-line options of default format
- Caption label format `brace' added

v3.2 (2011/07/30)
- Support of `beamer' document class improved
- Support of `magyar' babel option added
- Support of `sansmath' package added
- Support of `titletoc' package added to \DeclareCaptionType & \DeclareCaptionSubType
- Support of `tocbasic' package added to \DeclareCaptionType
- New options calcmargin=, calcmargin*=, calcwidth=, and calcwidth*=
- New option listtype= added
- New option parboxrestore=partial/full
- New options within= & without
- Option slc= as abbreviation of singlelinecheck= added
- Pre-defined text format `empty' added
- New command \captionbox
- New command \phantomcaption
- New command \setcaptiontype as replacement for \captionsetup{type=...}
- New command \setcaptionsubtype as replacement for \captionsetup{subtype}
- "Hyperref support is turned off because hyperref has stopped early" is not a warning anymore but an information instead

v3.3 (2013/01/06)
- Revised handling of continued floats and sub-captions
- New option box= and appropriate command \DeclareCaptionBox
- New option list-entry= (see also endfloat package documentation)
- Support of multiple optional arguments added to \captionsetup (see bicaption package documentation)
- Adapted to the elsarticle document class
- Adapted to the current version of memhfixc package, provided by the memoir document class
- Fixed compatibility problem with breqn and nag packages
- Corrects incorrect load order hyperref-float now (needs hyperref v6.82q or newer)
- New switch \ifsinglelinecaption for usage inside own commands added


bicaption package
-----------------

v0.9 (2010/09/19)
- 1st published version (see also http://www.mrunix.de/forums/showthread.php?t=68312)

v1.0 (2011/09/03)
- Support for list entries added

v1.1 (2012/12/26)
- \captionmainlanguage and \selectcaptionlanguage added


ltcaption package
-----------------

v1.0 (2007/04/15)
- 1st version

v1.1 (2007/09/01)
- Adapted to the NTG document classes (Support of \CaptionLabelFont & \CaptionTextFont added)
- Adapted to the `floatrow' package by Olga Lapko
- New macro \LTcaptype
- New environment longtable*

v1.2 (2008/03/28)
- New skip \LTcapskip

v1.3 (2011/09/12)
- New macro \CaptionLabelSeparator

v1.4 (2013/06/01)
- Adapted to the memoir document class (v3.7b)


subcaption package
------------------

v1.0 (2008/03/16)
- 1st published version

v1.1 (2011/08/17)
- New caption option subrefformat=
- New command \phantomsubcaption


newfloat package
----------------

v1.0 (2011/10/30)
- 1st published version

v1.1 (2013/04/27)
- New command \PrepareListOf


totalcount package
------------------

v1.0 (2008/03/09)
- 1st published version



==> README <==
README
------

  The subfigure package has been superseded by the subfig package.
  The reason for the name change is that the new subfig package is not
  exactly backward compatible with this package; although, it comes
  with a configuration file that *almost* allows backward
  compatibility, the difference is that exact spacing and layout of
  the subfloats are not preserved.

  The newer (subfig) package is an improvement over this package and
  although this package will continue to be supported, it will no longer
  be updated.

This directory contains version 2.1.5 of the subfigure package.
Use `make' to extract the subfigure package and run the local tests.

MANIFEST:
---------
Makefile           UNIX makefile to extract the subfigure package
                       and related material.
README             This file.
subfigure.dtx      The documented subfigure package.
subfigure.ins      The subfigure package installation file.
subfigure.pdf      Subfigure package documentation (as PDF).
test.tex           Test one: Mixed tables and figures.
test2.tex          Test two: Check for extra space around figure
test3.tex          Test four: Test of optional args and \subref.
test4.tex          Test four: Test of interaction with hyperref.
test5.tex          Test five: Test for class \let of \endfigure, etc.

FILES AFTER `make':
-------------------
Makefile           UNIX makefile to extract the subfigure package
                       and related material.
README             This file.
ltxdoc.cfg         Configuration file to print change history and
                       index on the subfigure package documentation.       
subfigure.cfg      Set the preferred options for subfigure version 2.1.
subfigure.dtx      The documented subfigure package.
subfigure.ins      The subfigure package installation file.
subfigure.pdf      Subfigure package documentation (as PDF).
subfigure.ps       Subfigure package documentation (as PostScript).
subfigure.sty      The subfigure package 
test.ps            Results of test one.
test.tex           Test one: Mixed tables and figures.
test2.ps           Results of test two.
test2.tex          Test two: Check for extra space around figure
test3.ps           Results of test three.
test3.tex          Test four: Test of optional args and \subref.
test4.pdf          Results of test four.
test4.tex          Test four: Test of interaction with hyperref.
test5.tex          Test five: Test for class \let of \endfigure, etc.
test5a.ps          Results of test five (log file).
test5b.ps          Results of test five (output).

NOTES:
------

By default, the subfigure.sty file acts like the older versions of the
subfigure package.  To make the preferred options default move the
subfigure.cfg file into the standard TEXINPUTS path along with the
subfigure.sty file.  This reduces the whitespace around the subfigures
and subtables and sets the table style to have the captions and
subcaptions preceed the table and subtables.

